Optimizing Time Series Forecasting: A Comparative Study of Adam and Nesterov Accelerated Gradient on LSTM and GRU networks Using Stock Market data

Several studies have discussed the impact different optimization techniques in the context of time series forecasting across different Neural network architectures. This paper examines the effectiveness of Adam and Nesterov's Accelerated Gradient (NAG) optimization techniques on LSTM and GRU neural networks for time series prediction, specifically stock market time-series. Our study was done by training LSTM and GRU models with two different optimization techniques - Adam and Nesterov Accelerated Gradient (NAG), comparing and evaluating their performance on Apple Inc's closing price data over the last decade. The GRU model optimized with Adam produced the lowest RMSE, outperforming the other model-optimizer combinations in both accuracy and convergence speed. The GRU models with both optimizers outperformed the LSTM models, whilst the Adam optimizer outperformed the NAG optimizer for both model architectures. The results suggest that GRU models optimized with Adam are well-suited for practitioners in time-series prediction, more specifically stock price time series prediction producing accurate and computationally efficient models. The code for the experiments in this project can be found at https://github.com/AhmadMak/Time-Series-Optimization-Research Keywords: Time-series Forecasting, Neural Network, LSTM, GRU, Adam Optimizer, Nesterov Accelerated Gradient (NAG) Optimizer

==> references.tex <==
\begin{thebibliography}{99}

\bibitem{nesterov1983method}
Yurii Nesterov.
\newblock A method for unconstrained convex minimization problem with the rate of convergence O (1/k2).
\newblock In {\em Dokl. Akad. Nauk. SSSR}, volume 269, pages 543, 1983.

\bibitem{kingma2014adam}
D. P. Kingma and J. L. Ba.
\newblock Adam: A Method for Stochastic Optimization.
\newblock In {\em 3rd International Conference on Learning Representations, ICLR 2015 - Conference Track Proceedings}, 2014.
\newblock \url{https://arxiv.org/abs/1412.6980v9} (Accessed: Aug. 17, 2024).

\bibitem{heaton2018deep}
J. Heaton.
\newblock Ian Goodfellow, Yoshua Bengio, and Aaron Courville: Deep learning: The MIT Press, 2016, 800 pp, ISBN: 0262035618.
\newblock {\em Genet Program Evolvable Mach}, 19(1–2):305–307, 2018.

\bibitem{ruder2016overview}
S. Ruder.
\newblock An overview of gradient descent optimization algorithms.
\newblock {\em arXiv preprint arXiv:1609.04747}, 2016.
\newblock \url{https://arxiv.org/abs/1609.04747v2} (Accessed: Aug. 17, 2024).

\bibitem{hewamalage2021recurrent}
H. Hewamalage, C. Bergmeir, and K. Bandara.
\newblock Recurrent Neural Networks for Time Series Forecasting: Current status and future directions.
\newblock {\em Int J Forecast}, 37(1):388–427, 2021.
\newblock \doi{10.1016/J.IJFORECAST.2020.06.008}.

\bibitem{brownlee2018deep}
Jason Brownlee.
\newblock Deep Learning for Time Series Forecasting: Predict the Future with MLPs ... - Jason Brownlee - Google Books.
\newblock Machine Learning Mastery, 2018.
\newblock \url{https://books.google.com.ng/books/about/Deep_Learning_for_Time_Series_Forecastin.html?id=o5qnDwAAQBAJ&redir_esc=y} (Accessed: Aug. 17, 2024).

\bibitem{sutskever2013importance}
I. Sutskever, J. Martens, G. Dahl, and G. Hinton.
\newblock On the importance of initialization and momentum in deep learning.
\newblock In {\em PMLR}, 2013.
\newblock \url{https://proceedings.mlr.press/v28/sutskever13.html} (Accessed: Aug. 19, 2024).

\bibitem{bengio2012advances}
Y. Bengio, N. Boulanger-Lewandowski, and R. Pascanu.
\newblock Advances in Optimizing Recurrent Networks.
\newblock In {\em ICASSP, IEEE International Conference on Acoustics, Speech and Signal Processing - Proceedings}, pages 8624–8628, 2012.
\newblock \doi{10.1109/ICASSP.2013.6639349}.

\bibitem{reddi2019convergence}
S. J. Reddi, S. Kale, and S. Kumar.
\newblock On the Convergence of Adam and Beyond.
\newblock In {\em 6th International Conference on Learning Representations (ICLR)}, 2019.
\newblock \url{https://openreview.net/forum?id=ryQu7f-RZ}.

\bibitem{gers2003learning}
F. A. Gers, N. N. Schraudolph, and J. Schmidhuber.
\newblock Learning precise timing with LSTM recurrent networks.
\newblock {\em Journal of Machine Learning Research}, 3(1):115–143, 2003.
\newblock \doi{10.1162/153244303768966139}.

\bibitem{chung2014empirical}
J. Chung, C. Gulcehre, K. Cho, and Y. Bengio.
\newblock Empirical Evaluation of Gated Recurrent Neural Networks on Sequence Modeling.
\newblock In {\em Proceedings of the 27th International Conference on Neural Information Processing Systems (NeurIPS)}, 2014.
\newblock \url{https://arxiv.org/abs/1412.3555v1} (Accessed: Aug. 19, 2024).

\bibitem{qin2017dual}
Y. Qin, D. Song, H. Chen, W. Cheng, G. Jiang, and G. Cottrell.
\newblock A Dual-Stage Attention-Based Recurrent Neural Network for Time Series Prediction.
\newblock In {\em International Joint Conference on Artificial Intelligence (IJCAI)}, pages 2627–2633, 2017.

\bibitem{rasp2020weatherbench}
S. Rasp, P. D. Dueben, S. Scher, J. A. Weyn, S. Mouatadid, and N. Thuerey.
\newblock WeatherBench: A benchmark dataset for data-driven weather forecasting.
\newblock {\em Journal of Advances in Modelling Earth Systems}, 12(11), 2020.

\bibitem{kong2019residential}
W. Kong, Z. Y. Dong, Y. Jia, D. J. Hill, and Y. Xu.
\newblock Short-Term Residential Load Forecasting based on LSTM Recurrent Neural Network.
\newblock {\em IEEE Trans Smart Grid}, 10(1):841–851, 2019.

\bibitem{lim2020survey}
B. Lim and S. Zohren.
\newblock Time Series Forecasting With Deep Learning: A Survey.
\newblock {\em Philosophical Transactions of the Royal Society A}, 2020.

\bibitem{lai2018modeling}
Guokun Lai, Wei-Cheng Chang, Yiming Yang, and Hanxiao Liu.
\newblock Modeling Long- and Short-Term Temporal Patterns with Deep Neural Networks.
\newblock In {\em Proceedings of the 41st International ACM SIGIR Conference on Research and Development in Information Retrieval}, pages 95--104, 2018.

\bibitem{qiu2020stock}
J. Qiu, B. Wang, and C. Zhou.
\newblock Forecasting stock prices with long-short term memory neural network based on attention mechanism.
\newblock {\em PLoS One}, 15(1), 2020.
\newblock \doi{10.1371/journal.pone.0227222}.

\bibitem{zhou2020energy}
C. Zhou, et al.
\newblock Using long short-term memory networks to predict energy consumption of air-conditioning systems.
\newblock {\em Sustain Cities Soc}, 55:102000, 2020.
\newblock \doi{10.1016/J.SCS.2019.102000}.

\bibitem{han2011data}
J. Han, M. Kamber, and J. Pei.
\newblock {\em Data Mining: Concepts and Techniques}, 3rd ed.
\newblock Morgan Kaufmann, 2011.

\bibitem{abadi2016tensorflow}
Mart{\'\i}n Abadi, Ashish Agarwal, Paul Barham, Eugene Brevdo, Zhifeng Chen, Craig Citro, Greg S. Corrado, Andy Davis, Jeffrey Dean, Matthieu Devin, and others.
\newblock Tensorflow: Large-scale machine learning on heterogeneous distributed systems.
\newblock {\em arXiv preprint arXiv:1603.04467}, 2016.

\bibitem{szegedy2016rethinking}
Christian Szegedy, Vincent Vanhoucke, Sergey Ioffe, Jon Shlens, and Zbigniew Wojna.
\newblock Rethinking the inception architecture for computer vision.
\newblock In {\em Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 2818--2826, 2016.

\bibitem{bergstra2012random}
James Bergstra and Yoshua Bengio.
\newblock Random search for hyper-parameter optimization.
\newblock {\em Journal of machine learning research}, 13(2), 2012.

\bibitem{bottou2010large}
L{\'e}on Bottou.
\newblock Large-scale machine learning with stochastic gradient descent.
\newblock In {\em Proceedings of COMPSTAT'2010: 19th International Conference on Computational Statistics, Paris France, August 22-27, 2010 Keynote, Invited and Contributed Papers}, pages 177--186, 2010.
\newblock Springer.

\bibitem{cho2014learning}
Kyunghyun Cho, Bart van Merrienboer, Caglar Gulcehre, Dzmitry Bahdanau, Fethi Bougares, Holger Schwenk, and Yoshua Bengio.
\newblock Learning Phrase Representations using RNN Encoder-Decoder for Statistical Machine Translation.
\newblock In {\em Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 1724–1734, 2014.

\bibitem{witten2016data}
I. H. Witten, E. Frank, M. A. Hall, and C. J. Pal.
\newblock {\em Data Mining: Practical Machine Learning Tools and Techniques}, 4th ed.
\newblock Morgan Kaufmann, 2016.

\bibitem{smola2004kernels}
A. J. Smola and B. Sch{\"o}lkopf.
\newblock A tutorial on support vector regression.
\newblock {\em Statistics and Computing}, 14(3):199–222, 2004.
\newblock \doi{10.1023/B:STCO.0000035301.49000.88}.

\end{thebibliography}

